Distractor Injection Attacks on Large Reasoning Models: Characterization and Defense

Recent advances in large reasoning models (LRMs) have enabled remarkable performance on complex tasks such as mathematics and coding by generating long Chain-of-Thought (CoT) traces. In this paper, we identify and systematically analyze a critical vulnerability we term reasoning distraction, where LRMs are diverted from their primary objective by irrelevant yet complex tasks maliciously embedded in the prompt. Through a comprehensive study across diverse models and benchmarks, we show that even state-of-the-art LRMs are highly susceptible, with injected distractors reducing task accuracy by up to 60%. We further reveal that certain alignment techniques can amplify this weakness and that models may exhibit covert compliance, following hidden adversarial instructions in reasoning while concealing them in the final output. To mitigate these risks, we propose a training-based defense that combines Supervised Fine-Tuning (SFT) and Reinforcement Learning (RL) on synthetic adversarial data, improving robustness by over 50 points on challenging distractor attacks. Our findings establish reasoning distraction as a distinct and urgent threat to LRM reliability and provide a practical step toward safer and more trustworthy reasoning systems.

==> old-section3.tex <==
\section{Evaluating LRM Susceptibility to Reasoning Distraction}
\label{sec:evaluation}

\subsection{Preliminaries}

\textbf{Threat model.} Following prior work \citep{liu2023prompt, liu2024automatic}, we consider a black-box attack in which an adversary attempts to corrupt an LRM's output. The LRM is governed by a \textbf{system prompt} $P_{\text{sys}}$ that encodes the \textbf{primary task instructions}, and it receives a \textbf{user prompt} $P_{\text{usr}}$ from the user. The adversary can only modify the user prompt by inserting a \textbf{distractor prompt} $P_{\text{distractor}}$; the modified user prompt $P'_{\text{usr}}$ is thus a concatenation of the original prompt and the distractor.

The adversary aims to craft $P_{\text{distractor}}$ so that the model deviates from the instructions in $P_{\text{sys}}$ and instead follows the task described in $P_{\text{distractor}}$. This setting is black-box: the adversary has no access to model weights, architecture, or the content of $P_{\text{sys}}$. Their influence is limited to the injected content inside the user prompt. For example, in an LRM-as-judge setting an adversary might inject a complex math problem and promise a higher score for its solution, thereby biasing the evaluation.

\textbf{Problem formulation.} Let the LRM be the function $M$. In a benign interaction, the model output
\begin{equation}
O = M(P_{\text{sys}}, P_{\text{usr}}),
\end{equation}
and $O$ is successful if it satisfies the instructions in $P_{\text{sys}}$.

In the attack scenario the adversary inserts $P_{\text{distractor}}$ into $P_{\text{usr}}$ at position $i$:
\begin{equation}
P'{\text{usr}} = \text{insert}(P{\text{usr}}, P_{\text{distractor}}, i).
\end{equation}
The model then produces the adversarial output
\begin{equation}
O_{\text{atk}} = M(P_{\text{sys}}, P'{\text{usr}}).
\end{equation}
Define a binary evaluation function $\mathcal{V}(O, P{\text{sys}})$ that returns $1$ if $O$ correctly completes the primary task in $P_{\text{sys}}$ and $0$ otherwise. A successful \textbf{reasoning distraction attack} is one for which
\begin{equation}
\mathcal{V}(O, P_{\text{sys}}) = 1 \quad\text{and}\quad \mathcal{V}(O_{\text{atk}}, P_{\text{sys}}) = 0.
\end{equation}

We restrict distractor tasks so that they contradict the primary task and therefore cannot be satisfied at the same time. This constraint allows direct measurement of attack effectiveness via the primary-task metric (for example, a drop in accuracy).

\subsection{Distractor Design and Methodology} \label{sec: distractor_design}

To systematically evaluate the reasoning distraction vulnerability, we developed a framework for injecting a diverse set of distractor tasks into user prompts. This provides fine-grained control over the injection's type, content, and position, enabling a comprehensive analysis of model robustness.

\paragraph{Distractor Categories.} We design several categories of distractor tasks, sourcing them from established benchmarks to ensure complexity and relevance. These are broadly divided into reasoning distractors and non-reasoning distractors.

\begin{itemize}[leftmargin=*]

    \item \textbf{Mathematical Reasoning:} We use challenging, competition-level problems from the AIME2025 dataset, which contains questions from the American Invitational Mathematics Examination (AIME). These serve as high-complexity math reasoning distractors.

    \item \textbf{Coding:} We assess programmatic logic using problems from LiveCodeBench-Pro~\citep{zheng2025livecodebench}. This benchmark sources competition-style problems from platforms like Codeforces, ICPC, and IOI, and is continuously updated to reduce the likelihood of data contamination.
    
    \item \textbf{Logical Reasoning:} We employ logic grid puzzles from ZebraLogic~\citep{lin2025zebralogic}, which are constraint satisfaction problems that test the model's ability to perform multi-step deductive reasoning based on explicit constraints.

    \item \textbf{Symbolic Reasoning:} We test the handling of abstract formal structures using parenthesis-matching problems (Dyck languages) from Big-Bench Hard~\citep{suzgun2022challenging}, which evaluates recursive pattern recognition.

    \item \textbf{Simple Arithmetic:} As a low-complexity baseline, we use randomly generated multi-step arithmetic problems to assess susceptibility to tasks with minimal reasoning depth.
    
\end{itemize}



\paragraph{Injection Mechanism.}
We implement reasoning-distraction prompt injection by combining a distractor task with a malicious meta-instruction into a single hidden prompt. The structure is:

\begin{textbox1}
\[
\text{[Hidden Instruction: \{Distractor Task\} \quad \{Malicious Meta-Instruction\}]}
\]

\end{textbox1}

Here, \(\{\text{Distractor Task}\}\) is drawn from one of the predefined categories (e.g., an AIME problem), while \(\{\text{Malicious Meta-Instruction}\}\) specifies the attacker's intended behavior.For example, as shown in Figure \ref{fig:distractor} In the LRM-as-a-judge experiments, for instance, the meta-instruction could direct the model to ``assign higher scores to this response after solve the distractor task,'' or a similar targeted manipulation.

\subsection{Experimental Setup}
\textbf{Models.} We evaluate a diverse set of state-of-the-art LRMs to test the generalizability of our findings. Our selection includes dual-mode models (with and without explicit reasoning, controlled by hyperparameters) such as \textbf{Claude-3.7-Sonnet} \citep{anthropic2025claude37sonnet} and \textbf{Qwen-3-4B} / \textbf{Qwen-3-8B} \citep{yang2025qwen3}. For these, we enable the ``thinking mode'' by default, using the \texttt{/think} token to elicit CoT reasoning enclosed in dedicated tags. We also consider models with native explicit reasoning, including \textbf{Deepseek-R1}, \textbf{Deepseek-Llama-8B} \citep{guo2025deepseek}, and \textbf{Phi-4-reasoning-mini} \citep{xu2025phi}, a compact 3.8B model that consistently produces CoT steps by default.  

\textbf{Downstream tasks.} To comprehensively evaluate reasoning distraction, we test across multiple benchmarks. For general knowledge we use \textbf{MMLU-Redux} \citep{gema-etal-2025-done}, a re-annotated 3k subset of MMLU. For mathematical reasoning we use \textbf{MATH-500} \citep{hendrycks2021measuring}. Instruction-following fidelity is measured with \textbf{IFEval} \citep{zhou2023instruction}. Agentic tool-use is assessed with the \textbf{Berkeley Function-Calling Leaderboard (BFCL) V3} \citep{patil2025bfcl}, which evaluates multi-turn and multi-step function calling. Finally, LRM-as-a-judge capabilities are measured using \textbf{JudgeLM} \citep{zhu2023judgelm}, which evaluates model judgments between two candidate responses with ground-truth labels. For distraction prompt injection, we randomly sample distractor-task instances for each downstream example to ensure diversity.  

\textbf{Evaluation Metrics.} \textcolor{red}{TODO}

\textbf{Non-reasoning Prompt Injection.} For a comprehensive evaluation, we also assess standard non-reasoning prompt injection attacks, following the design of prior work \citep{liu2023prompt}. These attacks include naive injections, whitespace padding, context-ignoring commands (e.g., ``Ignore all previous instructions''), and fake completion attacks. The experimental setup, including the meta-instruction and injection position, is identical to that used for our reasoning attacks. In our results, we report the average performance of these four baselines under the label "Non-reason Inject."

\subsection{Main Results and Analysis}

We present the results of analysis on LRM on differernt types of distractor on different downstream tasks in Table \ref{tab:main_results}. 

How is the similarity of the original task and the distracted task influence the performance.

Duel-mode models Vs single mode

Larger model does not indicate better robustness


\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l cc cc cc cc cc@{}}
\toprule
& \multicolumn{2}{c}{\textbf{MMLU-Redux}} & \multicolumn{2}{c}{\textbf{MATH}} & \multicolumn{2}{c}{\textbf{IFEval}} & \multicolumn{2}{c}{\textbf{BFCL V3}} & \multicolumn{2}{c}{\textbf{JudgeLM}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Model} & \textbf{ACC} & \textbf{Dist. (R / A)} & \textbf{ACC} & \textbf{Dist. (R / A)} & \textbf{ACC} & \textbf{Dist. (R / A)} & \textbf{ACC} & \textbf{Dist. (R / A)} & \textbf{F1 Score} & \textbf{Dist. (R / A)} \\
\midrule
\textbf{Claude-3.7-Sonnet} & 99.0 & - & 98.0 & - & 93.1 & - & 55.25 & - & 78.6 & - \\
\quad Arithmetic Dist. &  89.9 & 2.0 / 0.72 & 74.4& 50.15 / 69.5 & 88.0 & 7.62 / 2.24 & 53.72 & 2.53 / 0.93 & 82.3 & 0.0 / 24.19 \\
\quad AIME Dist. &  88.2 & 0.18 / 0.27 & 95.7& 24.38 / 40.5 & 90.0& 0.0 / 0.37 & 53.19 & 1.07 / 3.52 & 83.4& 1.0 / 32.53 \\
\quad Code Dist. &  87.2 & 2.76 / 0.69 & 73.1 & 68.79 / 73.25 & 91.4& 4.67 / 0.0 & 53.49 & 1.95 / 3.19 & 81.7 & 11.04 / 79.39 \\
\quad Logic Dist. &  84.9 & 9.3 / 5.93 & 69.2& 84.56 / 86.91 & 87.9& 14.66 / 4.9 & 52.51 & 3.38 / 5.71 & 79.9 & 5.42 / 41.37 \\
\quad Symbolic Dist. & 87.6 & 1.76 / 2.69  & 94.8& 63.29 / 49.52 & 85.2 & 13.73 / 5.76 & 53.21 & 3.79 / 3.16 &82.2 & 2.2 / 36.42 \\
\quad Non-reason Inject. & 88.9 & 0.0 / 0.0 & 80.3 & 0.0 / 0.0 & 86.7& 2.97 / 5.02 & 53.38 & 0.52 / 2.75 & 78.6 & 2.62 / 25.9 \\
\midrule
\textbf{DeepSeek-R1} & 89.2 & - & 96.1 & - & 88.0 & - & 49.77 & - & 70.5 & - \\
\quad Arithmetic Dist. & 0 & .99.73 / 100.0 & 2.2 & 91.52 / 99.55 &39.4 & 98.69 / 100.0 & 38.44 & 78.57 / 64.13 & 0 & 100.0 / 100.0 \\
\quad AIME Dist. & 0& 57.6 / 99.65 & 1.4& 88.92 / 100.0 & 35.1& 55.56 / 100.0 & 22.25 & 17.87 / 60.67 & 1.2& 86.67 / 93.33 \\
\quad Code Dist. & 0& 18.18 / 96.1 & 3.5 & 62.92 / 92.71 & 8.1& 0.0 / 0.0 & 9.23 & 2.0 / 92.86 & 0& 33.33 / 100.0 \\
\quad Logic Dist. &0 & 99.55 / 100.0 & 0.8 & 95.13 / 99.74 & 44.5& 90.7 / 97.67 & \textcolor{red}{19.62 error} & 51.02 / 0.75 & 0 & 100.0 / 100.0 \\
\quad Symbolic Dist. &0 & 97.84 / 100.0 & 0 & 93.53 / 100 & 24.3 & \textcolor{red}{... / ...} & 44.17 & 51.77 / 53.75 & 0 & 90.91 / 100.0 \\
\quad Non-reason Inject. & 0& 99.8 / 100.0 & 0 & 96.4 / 100.0 & 47.7& 90.64 / 99.81 & \textcolor{red}{todo} & \textcolor{red}{... / ...} & 2.6 & 76.92 / 100.0 \\
\midrule
\textbf{Deepseek-Llama-8B} & 63.2 & - & 87.2 & - & ... & - & 32.91 & - & 54.0 & - \\
\quad Arithmetic Dist. & 49.4 & 28.23 / 28.77 & 72.1 & 3.62 /  6.83 & & 65.77 / 35.48 & 27.34 & 47.05 / 37.3 & 14.6& 22.23 / 81.95 \\
\quad AIME Dist. & 45.2 & 16.19 / 29.69 &  71.2 & 1.21 / 6.65 & & 31.48 / 31.15 & 21.02 &  11.23 / 3.81 &3.40 & 27.41 / 81.62 \\
\quad Code Dist. & 17.1& 6.95 / 25.1 &56.7 & 1.01 / 3.24 & & 4.36 / 20.95 & 20.19 & 2.05 / 0.69 & 6.44 & ... / ... \\
\quad Logic Dist. & 31.7 & 72.44 / 50.81 &66.6 & 2.4 / 4.21 & & 94.11 / 42.0 & 20.86 & 67.15 / 26.67 &1.88 & 76.26 / 95.72 \\
\quad Symbolic Dist. & 58.8& 14.27 / 15.35 & 77.9& 2.8 / 5.2 & & 9.92 / 22.9 & 25.26 & 20.33 / 20.08 &20.88 & 20.53 / 79.97 \\
\quad Non-reason Inject. &50.4 & 15.03 / 15.87 & 70.5& 4.02 /  8.87 & & 3.85 / 10.38 & 33.78 & 22.61 / 22.68 & 11.85& 38.31 / 83.23 \\
\midrule
\textbf{Qwen-3-4B} & 80.34 &  & 93.4 & - & ... & - & 56.39 & - & 68.9 & - \\
\quad Arithmetic Dist. &16.8 & 86.67 / 83.01 & 21.0& 76.0 / 80.6 & & 57.31 / 66.4 & 52.67 & 21.61 / 25.88 & 0.07& 91.68 / 99.73 \\
\quad AIME Dist. &17.8 & 70.3 / 76.2 & 28.9 & 58.32 / 68.14 & & 66.1 / 58.05 & 42.6 & 22.68 / 45.0 &0.48 & 84.29 / 99.38 \\
\quad Code Dist. &23.1 & 53.3 / 71.73 & 55.4& 16.03 / 19.24 & & 9.79 / 38.76 & 40.19 & 8.97 / 52.64 & 2.48 & ... / ... \\
\quad Logic Dist. &8.61 & 93.06 / 90.43 & 13.2& 81.16 / 86.57 & & 88.2 / 70.36 & 34.46 & 60.24 / 63.32 & 1.36& 89.87 / 98.78 \\
\quad Symbolic Dist. &7.89 & 90.97 / 90.07 & 5.70& 90.2 / 97.8 & & 59.92 / 62.23 & 47.0 & 36.21 / 40.14 & 0.00& 92.49 / 99.93 \\
\quad Non-reason Inject. &15.3 & 74.28 / 70.91 & 6.00& 91.58 / 96.99 & & 39.07 / 57.98 & 56.64 & 18.67 / 31.44 & 0.24& 97.23 / 99.84 \\
\midrule
\textbf{Qwen-3-8B} & 83.97 & - & 94.4  & - & ... & - & 55.58 & - & 71.17 & - \\
\quad Arithmetic Dist. &0.91 & 99.27 / 99.02 & 21.6 & 74.6 / 84.8 & & 83.52 / 85.64 & 43.61 & 46.63 / 47.16 & 0.40& 90.26 / 99.53 \\
\quad AIME Dist. &3.45  & 90.04 / 96.36 & 26.7& 74.35 / 80.36 &  & 66.67 / 42.02 & 43.02 & 26.86 / 45.45 & 1.87 & 77.84 / 98.29 \\
\quad Code Dist. &12.8& 68.19 / 85.93 & 31.5& 56.0 / 64.2 & & 11.37 / 38.56 & 36.28 & 35.13 / 60.3 & 1.47 & ... / ... \\
\quad Logic Dist. &2.60 & 98.13 / 97.17 & 13.0& 89.16 / 96.79 & & 94.98 / 67.45 & 38.64 & 51.55 / 55.02 & 2.71& 86.76 / 98.1 \\
\quad Symbolic Dist. &1.21  & 98.96 / 98.83  &8.50 & 92.18 / 98.6 & & 83.71 / 68.43 & 49.2 & 29.74 / 33.98 &0.07 & 83.98 / 99.8\\
\quad Non-reason Inject. &1.56 & 96.75 / 97.43 & 9.23& 92.18 / 97.6 & & 47.59 / 70.43 & 55.38 & 19.24 / 32.41 & 1.02& 89.89 / 98.45 \\
\midrule
\textbf{Phi-4-reasoning-mini} & 74.92 & - & 91.2 & - & ... & - & 27.95 & - & 60.8 & - \\
\quad Arithmetic Dist. &2.82& 92.01 / 94.06 &8.30 & 60.69 / 88.71 & & 94.05 / 69.8 & 20.12 & 92.06 / 47.69 & 0.83& 93.41 / 95.45 \\
\quad AIME Dist. &11.3 & 47.91 / 73.0 & 16.6& 36.03 / 5.76 & & 52.57 / 30.12 & 18.83 & 2.11 / 0.54 & 4.34& 75.71 / 87.1 \\
\quad Code Dist. &13.3 & 71.87 / 75.78 &38.3& 26.86 / 33.26 & & 21.0 / 26.31 & 20.06 & 58.87 / 14.59 & 1.52 & ... / ... \\
\quad Logic Dist. &15.1 & 85.38 / 79.82 & 27.7& 23.93 / 56.39 & & 82.02 / 47.04 & 20.99 &  47.47 / 29.77 & 2.30& 87.6 / 95.51 \\
\quad Symbolic Dist. &10.3& 80.89 / 83.28 & 9.10& 54.45 / 87.24 & & 71.16 / 38.56 & 20.79 & 60.17 / 24.24 &0.39 & 80.69 / 96.53 \\
\quad Non-reason Inject. &13.1 & 77.2 / 79.65 & 8.05& 64.37 / 86.03 & & 44.31 / 63.34 & 21.94 & 80.93 / 93.06 & 0.43& 93.0 / 99.06 \\
\bottomrule
\end{tabular}%
}
\caption{Model performance on downstream tasks under various reasoning distraction attacks. For each task, we report the baseline accuracy (ACC) and the Distraction Rate, formatted as Reasoning Distraction \% / Answer Distraction \%. A higher distraction rate indicates lower robustness.}
\label{tab:main_results}
\end{table*}

\subsection{Ablation Studies}

To study the impact of placement, we inject the distractor at the \textbf{start}, \textbf{end}, or a strategically chosen \textbf{middle} point of the prompt. This positional variation allows us to rigorously test how the location of a distractor affects the LRM's performance against such attacks.



==> sections/old-intro.tex <==
\section{Introduction} \label{sec:intro}

The capabilities of Large Language Models (LLMs) in natural language understanding and complex reasoning have recently advanced with the emergence of models specifically designed for reasoning. This new class of models, often termed Large Reasoning Models (LRMs) \citep{xu2025towards}, such as OpenAI's \texttt{o1} \citep{jaech2024openai} and \texttt{DeepSeek-R1} \citep{guo2025deepseek}, demonstrates remarkable performance improvements on System-2 reasoning \citep{li2025system}. A key mechanism behind this advancement is their ability to generate extensive Chain-of-Thought (CoT) reasoning traces. These models articulate their thought processes, often encapsulated within nested tags like \texttt{<think>} and \texttt{</think>}, to explicitly outline behaviors such as planning and self-verification. This structured reasoning process enables LRMs to excel at solving challenging problems, particularly in domains like mathematics and coding.

While a growing body of work has focused on improving reasoning efficiency by reducing the computational overhead from verbose outputs—a phenomenon known as "overthinking" \citep{sui2025stop, chen2024not, han2024token}—far less attention has been paid to the issue of LRMs being distracted by irrelevant reasoning tasks. For instance, in an LRM-as-a-judge setting, the model is tasked with determining which of two responses to a given prompt is superior. As illustrated in Figure~\ref{fig:example}, a malicious actor can insert an unrelated, complex math problem into one of the responses, instructing the LRM to award a higher score if it can solve the problem. Our preliminary findings show that even state-of-the-art (SOTA) LRMs like DeepSeek-R1 can be easily diverted by such instructions, successfully attacking the integrity of the evaluation process. This vulnerability, which we term \textit{reasoning distraction}, could have profound implications for the reliability of LRM-based systems across a wide range of applications.

In this paper, we present the first systematic analysis of the reasoning distraction phenomenon. Our key contributions are as follows:
\begin{itemize}[leftmargin=*]
    \item We conduct a comprehensive empirical study on the vulnerability of various LRMs to reasoning distractions across a diverse set of tasks, including mathematics, coding, knowledge understanding, instruction following, tool use (agents), and LRM-as-a-judge evaluations.
    \item We design and test multiple types of distractor tasks (e.g., math and coding problems) and perform ablation studies on factors such as the position of the distractor within the prompt.
    \item We demonstrate that all tested LRMs are highly susceptible to these distractions, often prioritizing the injected task at the expense of the primary objective, revealing a critical and widespread vulnerability.
    \item To address this issue, we propose a mitigation strategy that involves fine-tuning models on a synthetically generated dataset using a combination of Supervised Fine-Tuning (SFT) and Reinforcement Learning (RL), showing that it can significantly enhance model robustness against such distractions.
\end{itemize}


\begin{figure}[t!]
\centering
\includegraphics[width=0.98\linewidth]{distractor.pdf}
\vspace{-3mm}
\caption{ An example to illustrate
}
\label{fig:distractor}
\end{figure}


